BrewCLIP: A Bifurcated Representation Learning Framework for Audio-Visual Retrieval

Previous methods for audio-image matching generally fall into one of two categories: pipeline models or End-to-End models. Pipeline models first transcribe speech and then encode the resulting text; End-to-End models encode speech directly. Generally, pipeline models outperform end-to-end models, but the intermediate transcription necessarily discards some potentially useful non-textual information. In addition to textual information, speech can convey details such as accent, mood, and and emphasis, which should be effectively captured in the encoded representation. In this paper, we investigate whether non-textual information, which is overlooked by pipeline-based models, can be leveraged to improve speech-image matching performance. We thoroughly analyze and compare End-to-End models, pipeline models, and our proposed dual-channel model for robust audio-image retrieval on a variety of datasets. Our approach achieves a substantial performance gain over the previous state-of-the-art by leveraging strong pretrained models, a prompting mechanism and a bifurcated design.

==> sections/tables/result_a2i.tex <==
\begin {table}[htb!]
\centering
\begin{center}
% \small
\caption{\textbf{Comparison of using ASR output vs ground truth in our zero-shot models}}
\label{tab:a2t}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{*{9}{c}}
\toprule                  
                            & \multicolumn{3}{c}{Speech2text} 
                            & \multicolumn{3}{c}{text2Speech}
                
                            \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Method & R1  & R5  & R10 & R1  & R5  & R10 \\
\midrule
Flickr8k & 33.6 & 57.7 & 68.0 & 53.9 & 77.8 & 85.4\\ 
SpokenCOCO & 33.6 & 57.7 & 68.0 & 53.9 & 77.8 & 85.4\\ 
LN-COCO & 2.4 & 10.1 & 17.7 & 10.0 & 26.1 & 36.1   \\
\bottomrule
\end{tabular}
}

\end{center}
\vspace{-11pt} 
\vspace{-4mm}
\end{table}

==> sections/tables/result_copy.tex <==
\section{Result}
\begin{table*}[hbt!]
\caption{\emph{Comparison with SoTA}}
\label{tab:result_SoTA}
\begin{adjustbox}{max width=1\textwidth,center}
% \centering
% \begin{tabular}{c c c c c c c c c c c c c c  c c c c c c c c c c c c c}
\begin{tabular}{*{25}{c}}
\toprule                  
                            & \multicolumn{12}{c}{Non-Spontaneous} 
                            & \multicolumn{12}{c}{Spontaneous}\\
                            \cmidrule(lr){3-12}\cmidrule(lr){15-24}
                            & \multicolumn{6}{c}{Flickr8k} 
                            & \multicolumn{6}{c}{SpokenCOCO}
                            & \multicolumn{6}{c}{LN-Flickr30k}
                            & \multicolumn{6}{c}{LN-COCO}
                            \\
                            \cmidrule(lr){3-6}\cmidrule(lr){9-12}\cmidrule(lr){15-18}\cmidrule(lr){21-24}
% \hline                 
                            & \multicolumn{3}{c}{Speech2Image} 
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{3}{c}{Speech2Image}
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{3}{c}{Speech2Image}
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{3}{c}{Speech2Image}
                            & \multicolumn{3}{c}{Image2Speech}
                            \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}\cmidrule(lr){23-25}
Method & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10\\
\midrule
Our experiments\\  
\midrule
Pipeline-only BrewCLIP(zero-shot) 
                    & 58.8 & 83.9 & 90.5 & 77.4 & 93.4 & 97.0  & - & - & - & - & - & - & - & - & - & - & - & - & 16.3 & 33.0 & 42.1 & 23.6 & 41.5 & 50.8  \\

Pipeline-only BrewCLIP (Prompted) 
                    & 68.5 & 89.9 & 94.5 & 80.8 & 95.8 & 98.6 & - & - & - & - & - & - & - & - & - & - & - & -  & 38.5 & 62.1 & 71.5 & 39.3 & 61.9 & 70.8
                    \\
BrewCLIP
                     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 40.4 & 66.8 & 76.9 & 42.4 & 67.6 & 77.2 
                    \\
\midrule
Previous approaches  \\
\midrule
SpeechCLIP-P 
                    & 39.1 & 72.0 & 83.0 & 54.5 & 84.5 & 93.2 & 35.8 & 66.5 & 78.0 & 50.6 & 80.9 & 89.1 & - & - & - & - & - & - & - & - & - & - & - & - \\
SpeechCLIP-C 
                    & 14.7 & 41.2 & 55.1 & 21.8 & 52.0 & 67.7 & 6.4 & 20.7 & 31.0 & 9.6 & 27.7 & 39.7 & - & - & - & - & - & - & - & - & - & - & - & - \\
ResDAVEnet 
                     & - & - & - & - & - & - & 17.3 & 41.9 & 55.0 & 22.0 & 50.6 & 65.2 & - & - & - & - & - & - & - & - & - & - & - & - \\
MILAN 

                     & 33.2 & 62.7 & 73.9 & 49.6 & 79.2 & 87.5 & - & - & - & - & - & - & 73.5 & - & 96.8 & 74.0 & - & 93.5 & - & - & - & - & - & -  \\
FaST-VGSco
                    & 26.6 & 56.4 & 68.8 & 36.2 & 66.1 & 76.5 &  31.8 & 62.5 & 75.0 & 42.5 & 73.7 & 84.9 & - & - & - & - & - & - & - & - & - & - & - & -  \\
FaST-VGSctf
                    &  29.3 & 58.6 & 71.0 & 37.9 & 68.5 & 79.9 & 35.9 & 66.3 & 77.9 & 48.8 & 78.2 & 87.0 & - & - & - & - & - & - & - & - & - & - & - & -  \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}
\vspace{100mm}
\subsection{Comparison with SoTA}
Benefited from the recently developed powerful pre-trained model, Whisper and CLIP. Our model with only the pipeline branch can perform zero-shot test by simply concatenating the ASR model Whisper and CLIP. As shown in table \ref{tab:result_SoTA}, the pipeline-only model under the zero-shot setting can significantly outperform existing works even if they are trained/fine-tuned in a fully supervised setting. And our well trained full model can even push the score further. 
To test our hypothesis that non-semantic information that only exist in utterance also plays an important role in audio-image retrieval task. We need to compare three variation of our model, which are pipeline-only model, e2e-only model and full model respectively. And we only ran the series of experiment on our selected spontaneous dataset LN-COCO. 

\vspace{100mm}
\begin{table*}[hbt!]
\caption{\emph{Comparison of different variations of our models}}
\label{tab:result_modeldif}
\begin{adjustbox}{max width=0.95\textwidth,center}
% \centering
% \begin{tabular}{c c c c c c c c c c c c c c  c c c c c c c c c c c c c}
\begin{tabular}{*{25}{c}}
\toprule                  
                            & \multicolumn{12}{c}{Non-Spontaneous} 
                            & \multicolumn{12}{c}{Spontaneous}\\
                            \cmidrule(lr){3-12}\cmidrule(lr){15-24}
                            & \multicolumn{6}{c}{Flickr8k} 
                            & \multicolumn{6}{c}{SpokenCOCO}
                            & \multicolumn{6}{c}{LN-Flickr30k}
                            & \multicolumn{6}{c}{LN-COCO}
                            \\
                            \cmidrule(lr){3-6}\cmidrule(lr){9-12}\cmidrule(lr){15-18}\cmidrule(lr){21-24}
% \hline                 
                            & \multicolumn{3}{c}{Speech2Image} 
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{3}{c}{Speech2Image}
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{3}{c}{Speech2Image}
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{3}{c}{Speech2Image}
                            & \multicolumn{3}{c}{Image2Speech}
                            \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}\cmidrule(lr){23-25}
Method & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10\\
\midrule
Our experiments\\  
\midrule
Pipeline-only BrewCLIP (Prompted) 
                    & 68.5 & 89.9 & 94.5 & 80.8 & 95.8 & 98.6 & - & - & - & - & - & - & - & - & - & - & - & -  & 38.5 & 62.1 & 71.5 & 39.3 & 61.9 & 70.8
                    \\
E2E-only BrewCLIP 
                    & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\                
BrewCLIP
                     & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 40.4 & 66.8 & 76.9 & 42.4 & 67.6 & 77.2 
                    \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}
\begin {table}[t!]
\centering
\begin{center}
% \small
\label{tab:ASR}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{*{9}{c}}
\toprule                  
                            & \multicolumn{3}{c}{Speech2Image} 
                            & \multicolumn{3}{c}{Image2Speech}
                            & \multicolumn{2}{c}{WER}
                            \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}
Method & R1  & R5  & R10 & R1  & R5  & R10 \\
\midrule
SpokenCOCO\\  
\midrule
ASR transcription \\
Ground truth \\
\midrule
LN-COCO\\  
\midrule
ASR transcription \\
Ground truth \\
\bottomrule
\end{tabular}
}
\caption{Comparison of using ASR output vs ground truth in our zero-shot models}
\end{center}
\vspace{-11pt} 
\vspace{-4mm}
\end{table}

\subsection{the impact of ASR result}

% \begin{table*}[t]
% \label{tab:result_ASR}
% \begin{adjustbox}{max width=0.5\textwidth}
% % \begin{tabular}{c c c c c c c c c c c c c c  c c c c c c c c c c c c c}
% \begin{center}
% \caption{Comparison of using ASR output vs ground truth in our zero-shot models}
% \resizebox{0.45\textwidth}{!}{%
% \begin{tabular}{*{9}{c}}
% \toprule                  
%                             & \multicolumn{3}{c}{Speech2Image} 
%                             & \multicolumn{3}{c}{Image2Speech}
%                             & \multicolumn{2}{c}{WER}
%                             \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}
% Method & R1  & R5  & R10 & R1  & R5  & R10 \\
% \midrule
% SpokenCOCO\\  
% \midrule
% ASR transcription \\
% Ground truth \\
% \midrule
% LN-COCO\\  
% \midrule
% ASR transcription \\
% Ground truth \\
% \bottomrule
% \end{tabular}}
% \end{center}
% \end{adjustbox}
% \end{table*}

% \begin{table*}[t]
% \caption{\emph{Comparison of different retrieval tasks with different methods on Flickr8k \\(CL: Contrastive loss, MHA: multi-head attention)}}
% \label{tab:flickr8k}
% \begin{adjustbox}{max width=1.1\textwidth,center}
% % \centering
% % \begin{tabular}{c c c c c c c c c c c c c c  c c c c c c c c c c c c c}
% \begin{tabular}{*{25}{c}}
% \toprule                  
%                             & \multicolumn{12}{c}{Non-Spontaneous} 
%                             & \multicolumn{12}{c}{Spontaneous}\\
%                             \cmidrule(lr){3-12}\cmidrule(lr){15-24}
%                             & \multicolumn{6}{c}{Flickr8k} 
%                             & \multicolumn{6}{c}{SpokenCOCO}
%                             & \multicolumn{6}{c}{LN-Flickr30k}
%                             & \multicolumn{6}{c}{LN-COCO}
%                             \\
%                             \cmidrule(lr){3-6}\cmidrule(lr){9-12}\cmidrule(lr){15-18}\cmidrule(lr){21-24}
% % \hline                 
%                             & \multicolumn{3}{c}{Speech2Image} 
%                             & \multicolumn{3}{c}{Image2Speech}
%                             & \multicolumn{3}{c}{Speech2Image}
%                             & \multicolumn{3}{c}{Image2Speech}
%                             & \multicolumn{3}{c}{Speech2Image}
%                             & \multicolumn{3}{c}{Image2Speech}
%                             & \multicolumn{3}{c}{Speech2Image}
%                             & \multicolumn{3}{c}{Image2Speech}
%                             \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}\cmidrule(lr){23-25}
% Method & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10 & R1  & R5  & R10\\
% % \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}\cmidrule(lr){23-25}
%  % \midrule
% % \multicolumn{19}{c}{End-to-End Model}  \\
%  % \midrule

 
% % e2e model without asr
% % whisper-clip-zero shot 
% % whipser-t5 - clip
% % whipser-clip- prompted
% % whisper-clip- shared prompted
% % whisper-clip-residual with hubert
% % shared prompt including hubert 
% \midrule
% Our experiments\\  
% \midrule
% Whisper-CLIP-zero-shot 
%                     & 58.8 & 83.9 & 90.5 & 77.4 & 93.4 & 97.0  & - & - & - & - & - & - & - & - & - & - & - & - & 16.3 & 33.0 & 42.1 & 23.6 & 41.5 & 50.8  \\
% % whipser-t5-clip 
% %                     & 14.7 & 37.2 & 50.6 & 24.1 & 50.0 & 64.1 & 28.1 & 52.6 & 63.9   & 35.6 & 64.9 & 76.6 & 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 & 71.9 &91.2 & 95.8 & 71.9 &91.2 & 95.8 \\
% % Whisper-CLIP-prompted 
% %                     & 14.7 & 37.2 & 50.6 & 24.1 & 50.0 & 64.1 & 28.1 & 52.6 & 63.9   & 35.6 & 64.9 & 76.6 & 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 & 71.9 &91.2 & 95.8 & 71.9 &91.2 & 95.8 \\
% Whisper-CLIP-bifurcated-zero-shot
%                     & 56.9 & 82.2 & 89.6 & 76.2 & 93.2 & 97.0 & - & - & - & - & - & - & - & - & - & - & - & - & 15.3 & 31.8 & 41.0 & 21.0 & 38.4 & 47.8
%                     \\
% Whisper-CLIP-bifurcated-linear
%                     & 54.8 & 83.1 & 90.7 & 69.1 & 93.1 & 97.7  & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -
%                     \\
% Whisper-CLIP-bifurcated-transformer
%                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 17.8 & 40.9 & 53.5 & 28.0 & 51.3 & 62.5 
%                     \\
%                     % & 54.2 & 83.5 & 90.9 & 68.7 & 93.9 & 97.8 
% Whisper-CLIP-shared-prompted-12-4 
%                     & 69.1 & 90.2 & 94.7 & 81.5 & 95.5 & 98.2 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% Whisper-CLIP-shared-prompted-1-4
%                     & 68.5 & 89.9 & 94.5 & 80.8 & 95.8 & 98.6 & - & - & - & - & - & - & - & - & - & - & - & -  & 38.5 & 62.1 & 71.5 & 39.3 & 61.9 & 70.8
%                     \\
% Whisper-CLIP-shared-prompted-1-4-audio-hubert
%                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 39.1 & 63.2 & 72.7 & 39.9 & 62.9 & 71.5  
%                     \\
% Whisper-CLIP-shared-prompted-1-4-not-shared-whisper-encoder
%                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 40.4 & 66.8 & 76.9 & 42.4 & 67.6 & 77.2 
%                     \\
% % Whisper-CLIP-shared-prompted-1-4-not-shared-whisper-encoder
% %                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 40.4 & 66.8 & 76.9 & 42.4 & 67.6 & 77.2 
% %                      \\
% e2e-hubert-transformer
%                      & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 10.2 & 27.7 & 39.3 & 13.4 & 32.2 & 43.6 
%                     \\

% % whisper-clip-residual 
% %                     & 14.7 & 37.2 & 50.6 & 24.1 & 50.0 & 64.1 & 28.1 & 52.6 & 63.9   & 35.6 & 64.9 & 76.6 & 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 & 71.9 &91.2 & 95.8 & 71.9 &91.2 & 95.8 \\
% \midrule
% Previous approaches  \\
% \midrule
% SpeechCLIP-P 
%                     & 39.1 & 72.0 & 83.0 & 54.5 & 84.5 & 93.2 & 35.8 & 66.5 & 78.0 & 50.6 & 80.9 & 89.1 & - & - & - & - & - & - & - & - & - & - & - & - \\
% SpeechCLIP-C 
%                     & 14.7 & 41.2 & 55.1 & 21.8 & 52.0 & 67.7 & 6.4 & 20.7 & 31.0 & 9.6 & 27.7 & 39.7 & - & - & - & - & - & - & - & - & - & - & - & - \\
% ResDAVEnet 
%                      & - & - & - & - & - & - & 17.3 & 41.9 & 55.0 & 22.0 & 50.6 & 65.2 & - & - & - & - & - & - & - & - & - & - & - & - \\
% MILAN 

%                      & 33.2 & 62.7 & 73.9 & 49.6 & 79.2 & 87.5 & - & - & - & - & - & - & 73.5 & - & 96.8 & 74.0 & - & 93.5 & - & - & - & - & - & -  \\
% FaST-VGSco
%                     & 26.6 & 56.4 & 68.8 & 36.2 & 66.1 & 76.5 &  31.8 & 62.5 & 75.0 & 42.5 & 73.7 & 84.9 & - & - & - & - & - & - & - & - & - & - & - & -  \\
% FaST-VGSctf
%                     &  29.3 & 58.6 & 71.0 & 37.9 & 68.5 & 79.9 & 35.9 & 66.3 & 77.9 & 48.8 & 78.2 & 87.0 & - & - & - & - & - & - & - & - & - & - & - & -  \\
% % Audio-Image CL(SpeechClip-P) - MHA - base 
% %                     &  29.1 & 59.9 & 72.5 & 40.5& 73.9 & 84.4 & 54.0 & 79.0 & 87.1 
% %                     &  63.1 & 88.2 & 93.8 & 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 &\\
% % Audio-Image CL(SpeechClip-P) - MHA - large 
% %                     & 48.0 & 78.7 & 87.3 & 64.2 & 90.5 & 95.4 & 90.8 & 98.3 & 99.1 & 93.9 & 99.4 & 99.8 & 61.8 & 85.8 & 92.2 & 78.0 & 93.7 & 96.8 &\\
% % % Trimodal CL - MHA - base 
% % %                     & 36.4 & 67.5 & 79.2 & 50.2 & 80.9 & 89.8 & 81.3 & 95.6 & 98.0 & 90.3 & 98.7 & 99.6& 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 &\\
% %  \midrule
% % \multicolumn{19}{c}{ASR Pipeline Model}  \\
% %  \midrule
% % Whisper-CL(CLIP) - zero shot  &  52.0 & 79.0 & 86.3 & 71.3 & 91.5 & 96.0 &- &- &- &- &- & - & - & - & - & - &- & - &\\
% % Wav2Vec-CL(CLIP)- zero shot - base &  46.8 & 73.5 & 81.4 & 67.3 & 88.5 & 93.2 &- &- &- &- &- & - & - & - & - & - &- & - &\\
% % Wav2Vec-CL(CLIP)- zero shot - large &  48.6 & 75.3 & 82.9 & 69.3 & 89.2 & 95.0 &- &- &- &- &- & - & - & - & - & - &- & - &\\
% % Wav2Vec-CL(CLIP)- fine tune - base &  50.1 & 78.36 & 86.06 & 69.4 & 89.9 & 94.6 &- &- &- &- &- & - & - & - & - & - &- & - &\\
% % %  \midrule
% % % \multicolumn{19}{c}{Text-Image Model}  \\
% % %  \midrule
% %  \midrule
% % \multicolumn{19}{c}{Previous approaches}  \\
% % \midrule
% % Text-Image CL(CLIP) - zero shot   
% %                     &  - & - &- &- &- &- &- &- &- &- &- & - & 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 &\\
% % % Text-Image CL(CLIP) - zero shot -default  
% % %                     &  - & - &- &- &- &- &- &- &- &- &- & - & 54.6 & 81.8 & 89.1 & 71.9 &91.2 & 95.8 &\\
% % % Text-Image CL(CLIP) - zero shot -reduced 
% % %                     &  - & - &- &- &- &- &- &- &- &- &- &- &17.3 &35.0 & 44.9 & 23.8 &44.7 & 56.1 &\\

% % % Hubert - Image-clip - linear - base  &  & \\
% % % Hubert - Image-clip - MLA & & \\
% % % Hubert - Text-clip - zero shot  &  & \\
% % % Trimodal & & \\
% % SpeechClip-C \cite{speechclip} & 8.2 & 25.7 & 37.2 & 14.1 & 34.5 & 49.2 &- &- &- &- &- &- & - & - & - & - & - & - & \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table*}


